Interactive Focus+Context Rendering for Hexahedral Mesh Inspection

The visual inspection of a hexahedral mesh with respect to element quality is difficult due to clutter and occlusions that are produced when rendering all element faces or their edges simultaneously. Current approaches overcome this problem by using focus on specific elements that are then rendered opaque, and carving away all elements occluding their view. In this work, we make use of advanced GPU shader functionality to generate a focus+context rendering that highlights the elements in a selected region and simultaneously conveys the global mesh structure in the surrounding. To achieve this, we propose a gradual transition from edge-based focus rendering to volumetric context rendering, by combining fragment shader-based edge and face rendering with per-pixel fragment lists. A fragment shader smoothly transitions between wireframe and face-based rendering, including focus-dependent rendering style and depth-dependent edge thickness and halos, and per-pixel fragment lists are used to blend fragments in correct visibility order. To maintain the global mesh structure in the context regions, we propose a new method to construct a sheet-based level-of-detail hierarchy and smoothly blend it with volumetric information. The user guides the exploration process by moving a lens-like hotspot. Since all operations are performed on the GPU, interactive frame rates are achieved even for large meshes.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> content/edge_rendering.tex <==
\section{Edge Rendering} \label{sec:EdgeRen}

The use of edge rendering has two purposes in our F+C implementation. On the one hand, we want to be able to show wireframe representation of the mesh via a possibly thinned-out mesh representation, which is built upon the LoD structure presented in \autoref{sec:lod}. On the other hand, we want to slightly accentuate edges in the context volume of faces that have an opacity not equal to zero.

\begin{figure}[tb]
 \centering
 \includegraphics[width=0.9\linewidth]{figures/edge/LineRenderingQuad.pdf}
 \caption{A sketch of the simplified edge rendering in the 2D case with quad faces. (a) A quad face is formed by four vertices. Two fragment positions are indicated as crosses inside of the face. The distance of the fragments to the edges are indicated as grey lines. (b) The edges are rendered as face-based lines using the point to line segment distance. Only one of the two indicated fragments lies close enough to the edge to get the line color. (c) Here, the result is shown that the viewer finally is presented. Outlines are drawn black (white in our program), but the individual line segments don't have a separator between them.}
 \label{fig:edge_rendering_quad}
\end{figure}

\begin{figure}[tb]
 \centering
 \includegraphics[width=0.9\linewidth]{figures/edge/LineRenderingArrow.pdf}
 \caption{A sketch of the simplified edge rendering in the 2D case with four quad faces. (a) Four edges meet in one vertex and form an arrow-like shape. (b) When making edges/lines invisible, unwanted holes appear in the arrow shapes. (c) An approach for closing these holes is ignoring lines with a low opacity in the calculation of the closest edge.}
 \label{fig:edge_rendering_arrow}
\end{figure}

For edge rendering, we present a single-pass face-based approach that is able to render both lines at the edges of faces and the volumetric saliency map. In \autoref{fig:edge_rendering_quad} and \autoref{fig:edge_rendering_arrow}, a sketch of this approach is shown in 2D. We render all faces of the mesh using a triangle representation. The vertex shader passes all vertices $v_0$, \textellipsis, $v_3$ of the face the triangle belongs to directly to the fragment shader. In the fragment shader, the fragment computes closest object-space distance to the face edges using the point to line segment distance. Finally, if the distance is less than the line width, it is colored using the color assigned to the edge. In our implementation, we have decided to assign the maximum attribute of all cells incident to the edge for the computation of color and opacity using the assigned transfer function. If no edge is in close proximity, the normal face color is used for pseudo volume rendering. In order to be able to discern edge and face colors, a different approach is used for the focus and context region. In the context region, the edge color gets slightly brightened. In the focus region, the edge color gets slightly darkened and a white outline. The outline rendering is similar to the depth-dependent halos proposed by Everts et al.~\cite{Everts:2009:TVCG}. The fragments belonging to the halo get assigned a larger depth value in order to make sure that only lines with a depth discontinuity get a halo effect.

In \autoref{fig:egde_rendering_context}, the user can see the rendering of the context region using pseudo volume rendering enhanced by edge rendering of highly opaque edges from a coarse mesh LoD, and a transparent wireframe enhancing the edge structure of the volume. Additionally, a white mesh outline is rendered improving the perception of the extent of the mesh. For this, the mesh boundary surface is rendered into a depth-buffer storing the depth of the closest fragments. Then, discontinuities in the depth buffer values are used to find boundary edges and interior edges on the boundary surface to improve the perception of the mesh structure. This way, both highly deformed mesh regions and the geometrical and topological structure of the mesh can be perceived more easily by the user.

\begin{figure}[tb]
 \centering

 \begin{tabular}{cccc}
 \hspace*{-0.9em}
 \subfloat[Pseudo volume rendering.]{\includegraphics[width=0.495\linewidth]{figures/edge/Edge_Rendering_Context_Volume.png}\label{fig:egde_rendering_context_volume}} \hspace*{-0.9em} &
 \subfloat[Enhanced context rendering.]{\includegraphics[width=0.495\linewidth]{figures/edge/Edge_Rendering_Context_Enhanced.png}\label{fig:egde_rendering_context_enhanced}}\\
 \end{tabular}
 \caption{The proposed context region rendering of the mesh in \autoref{fig:egde_rendering_context_enhanced} is comprised of the pseudo volume rendering and edge rendering. Model courtesy of Xu et al.~\cite{SingularityStructureSimplification2019}.}
 \label{fig:egde_rendering_context}
\end{figure}


==> content/volume_rendering.tex <==
\section{Pseudo Volume Rendering} \label{sec:VolRen}

\begin{figure}[tb]
 \centering

 \begin{tabular}{cccc}
 \hspace*{-0.9em}
 \subfloat[Opaque surfaces with wireframe.]{\includegraphics[width=0.495\linewidth]{figures/volume/Bunny_Surface.png}} \hspace*{-0.9em} &
 \subfloat[Volume rendering using distances traveled through cells.]{\includegraphics[width=0.495\linewidth]{figures/volume/Bunny_Volume_DistTraveled.png}\label{fig:vol_dist_traveled}}\\
 \hspace*{-0.9em}
 \subfloat[Pseudo face-based volume rendering using per-cell attributes for coloring.]{\includegraphics[width=0.495\linewidth]{figures/volume/Bunny_Volume_FacesPerCell.png}\label{fig:vol_per_cell}} \hspace*{-0.9em} &
 \subfloat[Pseudo face-based volume rendering using weighted per-vertex attributes for coloring.]{\includegraphics[width=0.495\linewidth]{figures/volume/Bunny_Volume_FacesPerAttribute.png}\label{fig:vol_per_attribute}}\\
 \end{tabular}
 \caption{Different possibilites of rendering volumetric saliency maps. The Jacobian ratio is mapped to a color and opacity. Model courtesy of Gregson et al.~\cite{HexMeshSGP2011}.}
 \label{fig:volume_rendering_types}
\end{figure}

In order to render the saliency maps indicating important mesh regions, an approach we call \textit{pseudo volume rendering} has been used. In \autoref{fig:volume_rendering_types}, different volume rendering approaches are compared to rendering the mesh using opaque surfaces.

For all shown models, the cell faces are converted to a triangle representation in a preprocess step and rendered into per-pixel linked lists \cite{Yang2010}. Per-pixel linked lists store all fragments that get rasterized into a certain pixel position in a first pass. In a final resolve pass, the fragments are sorted w.r.t.\ their depth and blended using front-to-back alpha blending. In our implementation, we use a GPU-friendly implementation of priority-queues introduced by Kern et al.~\cite{Kern:2020:TVCG}.

In \autoref{fig:vol_dist_traveled}, a standard volume rendering approach can be seen where the optical depth traveled through a cell is used to modulate the accumulated opacity along the view rays when using front-to-back alpha-blending \cite{RealTimeVol2006}. However, this approach has two major disadvantages. Firstly, when utilizing GPU rendering capabilities, we need to both rasterize front-faces as well as back-faces in order to be able to determine the distance traveled through a cell. This doubles the memory requirements for per-pixel linked lists, which is already very high, and quickly exceeds the available VRAM for high resolutions. Secondly, edges and the boundary of the mesh get blurred and the cell structure is lost when viewing the volume.

In \autoref{fig:vol_per_cell}, the cell front-faces are rendered with per-cell attributes, but without modulating the opacity using the optical depth. While this approach is considerably more performant, we get overestimated opacity and too hard edges in all regions where the view rays travel diagonally through neighboring elements. This effect is considerably improved in the approach shown in \autoref{fig:vol_per_attribute}, which we have decided to use as our \textit{pseudo volume rendering}. This is the approach does not use constant per-cell attributes, but volume-weighted per-vertex attributes for rendering. For computing the volume of the hexahedral cells, tetrakis hexahedra are assumed as defined by Grandy~\cite{Grandy:1997}. These attributes are then interpolated across the faces using the barycentric interpolation natively supported by graphics cards. For computing the attribute of a vertex, the attributes of all cells incident to an edge are weighted using the following formula.

\begin{equation}
\label{eqn:weighting-attributes}
a_{edge} = \frac{\sum_i{V_i \cdot a_i}}{\sum_i{V_i}}
\end{equation}

In case of the Jacobian ratio metric, the formula below is used.

\begin{equation}
\label{eqn:weighting-jacobian}
J_{edge} = \frac{\sum_i{V_i}}{\sum_i{\frac{V_i}{J_i}
}}
\end{equation}

While edges in \autoref{fig:vol_per_attribute} are already slightly accentuated, this effect is dependent on the viewing angle. In order to solve this problem, in our final focus+context approach edges are further accentuated using line rendering.
